Incremental Discovery of Prominent Situational Facts

We study the novel problem of finding new, prominent situational facts, which are emerging statements about objects that stand out within certain contexts. Many such facts are newsworthy---e.g., an athlete's outstanding performance in a game, or a viral video's impressive popularity. Effective and efficient identification of these facts assists journalists in reporting, one of the main goals of computational journalism. Technically, we consider an ever-growing table of objects with dimension and measure attributes. A situational fact is a "contextual" skyline tuple that stands out against historical tuples in a context, specified by a conjunctive constraint involving dimension attributes, when a set of measure attributes are compared. New tuples are constantly added to the table, reflecting events happening in the real world. Our goal is to discover constraint-measure pairs that qualify a new tuple as a contextual skyline tuple, and discover them quickly before the event becomes yesterday's news. A brute-force approach requires exhaustive comparison with every tuple, under every constraint, and in every measure subspace. We design algorithms in response to these challenges using three corresponding ideas---tuple reduction, constraint pruning, and sharing computation across measure subspaces. We also adopt a simple prominence measure to rank the discovered facts when they are numerous. Experiments over two real datasets validate the effectiveness and efficiency of our techniques.

==> alg/alg-baseline.tex <==
\begin{algorithm}[t]
\caption{\algname{BaselineSeq}}
\label{alg:baseline}
\LinesNumbered
\small

\SetKw{KwAnd}{and}
\SetKw{KwDownTo}{downto}

\KwIn{$R(\mathcal{M},\mathcal{D})$: existing tuples; $t$: the new tuple}

\KwOut{$S^t$: the contextual skylines for $t$}

\BlankLine

$S^t \leftarrow \emptyset$;

\ForEach{$M \subseteq \mathcal{M}$}
{
  $S \leftarrow \mathcal{C}^t$;~\label{line:initS}

  \ForEach{$t' \in R$~\label{line:comp}}
  {
    \lIf{$t \prec_M t'$}{$S \leftarrow S - \mathcal{C}^{t,t'}$;\label{line:subtract}}
  }
  \ForEach{$C \in S$~\label{line:include}}
  {
     $S^t \leftarrow S^t \cup \{(C,M)\}$;
  }
}
$R \leftarrow R \cup \{t\}$;

\Return{$S^t$};
\end{algorithm}


==> alg/alg-bottomup-dfs.tex <==
\begin{algorithm}[t]
\label{algo:Bottom_up dfs}
\caption{Bottom-up DFS algorithm to discover contextual skylines}
\LinesNumbered

\KwIn{$R$: existing set of tuples; $t$: new tuple; $\mathcal{C}^t$: contextual constraints specific to $t$.}

\KwOut{$\mathcal{S}$: where $\mathcal{S} = \{C : t \in \mu_M(\sigma_C(R \cup \{t\}))\}$}

\BlankLine

$Sackt.push(B^{\mathcal{C}^t})$;\\
\While{$Stack.empty()=false$}
{
	$C \leftarrow Stack.pop()$;\\	
	$C.visited \leftarrow true$;\\		
	$isDominated \leftarrow false$;\\
	\ForEach{$t' \in \mu_M(\sigma_C$ $(R)$}
	{
	    \If{$t \prec t'$}	
	    {
	    	$isDominated \leftarrow true$;\\
			$break$;
	    }
	    \ElseIf{$t' \prec t$}
	    {
			$\mu_M(\sigma_C$ $(R)).remove(t')$;	
	    }
	}
	\If{$isDominated=false$}
	{
		$\mu_M(\sigma_C$ $(R)).insert(t)$;\\	
		$S \leftarrow S \cup \{C\}$;\\
		\ForEach{$C' \in \mathcal{P}_C[t]$}
		{
			\If{$Stack.contain(C')=false\ \text{and}\ C'.visited=false$}
			{
				$Stack.push(C')$;
			}
		}
	}
}
\Return{$S$};	
\end{algorithm}

==> alg/alg-bruteforce.tex <==
\begin{algorithm}[t]
\caption{\algname{BruteForce}}
\label{alg:bruteforce}
\LinesNumbered
\small

\SetKw{KwAnd}{and}
\SetKw{KwDownTo}{downto}

\KwIn{$R(\mathcal{M},\mathcal{D})$: existing tuples; $t$: the new tuple}

\KwOut{$S^t$: the contextual skylines for $t$}

\BlankLine

$S^t \leftarrow \emptyset$;

\ForEach{$M \subseteq \mathcal{M}$}
{
  \ForEach{$C \in \mathcal{C}^t$}
  {
    $\mathit{pruned} \leftarrow \KwSty{false}$;

    \ForEach{$t' \in R$~\label{line:comp}}
    {
      \If{$t \prec_M t'$ \bf{and} $t' \in \sigma_{C}(R)$}
      {
        $\mathit{pruned} \leftarrow \KwSty{true}$;

        \KwSty{break};
      }
    }
    \lIf{{\bf not} $pruned$}{$S^t \leftarrow S^t \cup \{(C,M)\}$;}
  }
}
$R \leftarrow R \cup \{t\}$;

\Return{$S^t$};
\end{algorithm}


==> alg/alg-build-constraint.tex <==
\begin{algorithm}[t]
\caption{Find $\mathcal{C}^t$}
\label{alg:find-constraints}
\LinesNumbered
\small

\SetKw{KwAnd}{and}
\SetKw{KwDownTo}{downto}

\KwIn{$t \in R$}

\KwOut{$\mathcal{C}^t$: constraints satisfied by $t$}

\BlankLine
$\mathcal{C}^t \leftarrow \emptyset$;\\
$Q \gets \emptyset$; $Q.\mathit{enqueue}(\top)$;\\

\While{{\bf not} $Q.\mathit{empty}()$}
{
  $C \leftarrow Q.\mathit{dequeue}()$;\\
  $\mathcal{C}^t \leftarrow \mathcal{C}^t \cup \{C\}$;\\
  $i \leftarrow n$;\\
  \While{$i > 0$ \bf{and} $C.d_i = *$}
  {
    $C' \leftarrow C$;\\
    $C'.d_i \leftarrow t.d_i$;\\
    $Q.\mathit{enqueue}(C')$;\\
    $i \leftarrow i - 1$;\\
  } \label{line:whileloop}
}

\Return{$\mathcal{C}^t$};
\end{algorithm}


==> alg/alg-dominated.tex <==
\begin{algorithm}[t]
\label{alg:dominated}
\caption{\algname{Dominated}}
\LinesNumbered
\small

\BlankLine

\ForEach{$C' \in \mathcal{C}^{t,t'}$}
{
	$C'.pruned \leftarrow true$;
}

\end{algorithm}


==> alg/alg-dominates.tex <==
\begin{algorithm}[t]
\label{alg:dominates}
\caption{\algname{Dominates}}
\LinesNumbered
\small

\BlankLine

$\mu_{C,M}.remove(t')$;\\	
\ForEach{$C' \in \mathcal{CH}^{t'}_C-\mathcal{C}^{t}$}
{
	$stored \leftarrow false$;\\
	\ForEach{$C'' \in \mathcal{A}^{t'}_{C'}-\mathcal{C}^{t}$}
	{
	 	\If{$t' \in \mu_{C'',M}$}
	    {
	    	$stored \leftarrow true$;\\
	    	$break$;\\
	    }
	 }
	 \If{{\bf not} $stored$}
	 {
	 	$\mu_{C',M}.insert(t')$;\\
	 }	    			
}

\end{algorithm}


==> alg/alg-enqueue_children.tex <==
\begin{algorithm}[t]
\label{alg:enqueuechildren}
\caption{\algname{EnqueueChildren}}
\LinesNumbered
\small

\BlankLine

\ForEach{$C' \in \mathcal{CH}^t_C$}
{
	\If{{\bf not} $C.pruned$}
	{
		$C'.storedInAncestor \leftarrow true$;		
	}
	\If{$(${\bf not} $Q.contain(C'))$}
	{		
		$Q.enqueue(C')$;
	}
}	

\end{algorithm}


==> alg/alg-frontier-measure-subspace.tex <==
\begin{algorithm}[t]
\label{algo:frontier_measure_subspace}
\caption{Frontier algorithm for each measure subspace}
\LinesNumbered
\small

\BlankLine

\ForEach{$M \subseteq \mathcal{M}$}
{
	$count \leftarrow 0$\\
	\If{$i\ is\ a\ power\ of\ 2$}
	{
		$F_i \leftarrow TopDown()$
	}
	\Else
	{
		$F_i \leftarrow Frontier(F_{i-1})$\\
	}
	
	\ForEach{$C \in \mathcal{P}_{\bot(\mathcal{C}^t)}$}
	{
		\ForEach{$s \in F_i$}
		{
			\If{$s \in C \cup \mathcal{A}_{C}$}
			{
				$count \leftarrow count + 1$\\
				$break$\\
			}
		}
		\If{$count < |\bot(\mathcal{C}^t)|$}
		{
			$F_i \leftarrow F_i \cup \{\bot(\mathcal{C}^t)\}$\\
		}
	}
}
\end{algorithm}


==> alg/alg-frontier.tex <==
\begin{algorithm}[t]
\label{algo:frontier}
\caption{Frontier algorithm to derive frontier}
\LinesNumbered
\small

\KwIn{$R$: existing set of tuples; $t$: new tuple; $F_{i-1}: Frontier(M_{i-1})$.}

\KwOut{$F_i$: where $F_i = Frontier(M_i)$}

\BlankLine

$F1 \leftarrow \phi$;\\
$F2 \leftarrow \phi$;\\

$U \leftarrow \phi$;\\

\ForEach{$C \in F_{i-1}$}
{	
	$isDominating \leftarrow false$;\\
	\ForEach{$t' \in \lambda_{M_i}(\sigma_C$ $(R))$}
	{
	    \If{$t \prec t'$}	
	    {	    				
			$break$;
	    }
	    \ElseIf{$t' \prec t$}
	    {
		    $isDominating \leftarrow true$;\\
	    	$\lambda_{M_i}(\sigma_C$ $(R)).remove(t')$;\\	
	    	\ForEach{$C' \in \mathcal{CH}^{t'}_C$}
	    	{
	    		\If{$C' \notin \mathcal{C}^{t}$}
	    		{
	    			$\lambda_{M_i}(\sigma_{C'}$ $(R)).insert(t')$;
	    		}
	    	}
	    }
	}
	\If{$isDominating=false$}
	{
		$U \leftarrow U \cup \{C\}$;\\
	}
}
$F1 \leftarrow pullUp(U);$\\
$F2 \leftarrow pushDown(F_{i-1});$\\

\Return{$F1 \cup F2$};
\end{algorithm}


==> alg/alg-multidimensional-index.tex <==
\begin{algorithm}[t]
\label{alg:multidim}
\caption{\algname{BaselineIdx}}
\LinesNumbered
\small

\SetKw{KwAnd}{and}
\SetKw{KwDownTo}{downto}

\KwIn{$R(\mathcal{M},\mathcal{D})$: existing tuples; $t$: the new tuple; $idx$: multi-dimensional index over $R$}

\KwOut{$S^t$: the contextual skylines for $t$}

\BlankLine

$S^t \leftarrow \emptyset$;

\ForEach{$M \subseteq \mathcal{M}$}
{
  $S \leftarrow \mathcal{C}^t$;

  $R' \leftarrow$ range query on $idx$ to find tuples dominating $t$ in $M$;~\label{line:R}

  \ForEach{$t' \in R'$}
  {
	$S \leftarrow S - \mathcal{C}^{t,t'}$;
  }
  \ForEach{$C \in S$}
  {
    $S^t \leftarrow S^t \cup \{(C,M)\}$;
  }
}
$R \leftarrow R \cup \{t\}$;

$idx.insert(t)$;~\label{line:insertMI}

\Return{$S^t$};

\end{algorithm}


==> alg/alg-old-materialize.tex <==
%%% Chengkai Li (July 9 2012) : I am not sure when we discussed this algorithm and if this was ever implemented.

\begin{algorithm}[t]
\label{alg:mutual}
\caption{$contextual\_skyline(R,t,\mathcal{M})$: Materialization based algorithm to discover contextual skylines}
\LinesNumbered

\SetKw{KwAnd}{and}
\SetKw{KwDownTo}{downto}

\KwIn{$R$: existing set of tuples; $t$: new tuple; $\mathcal{M}$: where $\mathcal{M} = \{C:\mu_M\sigma_{C}(R)$ is materialized$\}$}

\KwOut{$\mathcal{S}$: where $\mathcal{S} = \{C : t \in \mu_M(\sigma_C(R \cup \{t\}))\}$}

\BlankLine

$\mathcal{S} \leftarrow tuple\_specific\_constraints(t)$;\\

$\mathcal{M} \leftarrow \mathcal{M} \cap \mathcal{S}$;\\

\ForEach{$C \in \mathcal{M}$}
{
  \ForEach{$t' \in \mu_M\sigma_{C}(R)$}
  {
    \If{$t' \succ t$}
    {
      $\mathcal{S} \leftarrow \mathcal{S} - \mathcal{C}^{t,t'}$;\\
      $\mathcal{M} \leftarrow \mathcal{M} - (\mathcal{M} \cap \mathcal{C}^{t,t'})$;\\
      \textbf{break} ;
    }
    \ElseIf{$t \succ t'$}
    {
      $\mu_M\sigma_{C}(R) \leftarrow \mu_M\sigma_{C}(R) - {t'}$;\\
      $\mu_M\sigma_{C}(R) \leftarrow \mu_M\sigma_{C}(R) \cup {t}$;\\
    }
  }
}

\ForEach{$C \in \mathcal{S}$}
{
  \ForEach{$t' \in \mathcal{T}^C$}
  {
    \If{$t' \succ t$}
    {
      $\mathcal{S} \leftarrow \mathcal{S} - \mathcal{C}^{t,t'}$;\\
      \textbf{break} ;
    }
  }
}

$R \leftarrow R \cup \{t\}$;

\Return{$\mathcal{S}$};

\end{algorithm}

==> alg/alg-partial-order-based.tex <==
\begin{algorithm}[t]
\label{alg:partial_order}
\caption{$contextual\_skyline(R, G(V,E), t, \mathcal{C}^t)$: Partial Order based algorithm to discover contextual skylines}
\LinesNumbered

\SetKw{KwAnd}{and}
\SetKw{KwDownTo}{downto}

\KwIn{$R$: existing set of tuples;\\ $G(V,E)$: a DAG representing $P$; $t$: new tuple; $\mathcal{C}^t$: contextual constraints specific to $t$.}

\KwOut{$\mathcal{S}$: where $\mathcal{S} = \{C : t \in \mu_M(\sigma_C(R \cup \{t\}))\}$}

\BlankLine

$\mathcal{S} \leftarrow \mathcal{C}^t$;

$Q \leftarrow \{t':t' \in V$ and indegree of $t' = 0\}$;

\While{$Q.empty()=false$}
{
  $t' \leftarrow dequeue(Q)$;

  \If{$t' \succ t$}
  {
    $\mathcal{S} \leftarrow \mathcal{S} - \mathcal{C}^{t,t'}$;\\
    $draw\_new\_edge \leftarrow true$;

    \ForEach{$t'' \in children(t')$}
    {
      $dominated = false$;\\
      \If{$t'' \succ t$}
      {
	$mark (t',t'') \, as \, visited$;	
	$draw\_new\_edge \leftarrow false$;
      }
      \ElseIf{$t'' \prec t$}
      {
	$dominated = true$;\\
	$remove \, edge (t',t'')$;\\
	\If{all $(x,t'') \in E$ are visited, where $x \in V$}
	{
	  $E \leftarrow E \cup \{(t,t'')\}$;
	}
      }
      \Else
      {
	$mark (t',t'') \, as \, visited$;
      }
      \If{$dominated = false$ $and$ all $(x,t'') \in E$ are visited, where $x \in V$}
      {
	$enqueue(Q,t'')$;
      }
    }
  }

  \Else
  {
    $draw\_new\_edge \leftarrow false$;\\
    \ForEach{$t'' \in children(t')$}
    {
      $mark (t',t'') \, as \, visited$;\\
      \If{$t'' \prec t$}
      {
	\If{all $(x,t'') \in E$ are visited, where $x \in V$}
	{
	  $E \leftarrow E \cup \{(t,t'')\}$;
	}
      }
      \Else
      {
	\If{all $(x,t'') \in E$ are visited, where $x \in V$}
	{
	  $enqueue(Q,t'')$;
	}
      }
    }
  }

  \If{$draw\_new\_edge = true$}
  {
    $E \leftarrow E \cup \{(t',t)\}$;
  }
}

$R \leftarrow R \cup \{t\}$;

\Return{$\mathcal{S}$};

\end{algorithm}

==> alg/alg-partition-based.tex <==
\begin{algorithm}[t]
\label{alg:partition}
\caption{$contextual\_skyline(R,t, \mathcal{C}^t)$: Partition based algorithm to discover contextual skylines}
\LinesNumbered

\SetKw{KwAnd}{and}
\SetKw{KwDownTo}{downto}

\KwIn{$R$: existing set of tuples; $t$: new tuple; $\mathcal{C}^t$: contextual constraints specific to $t$.}

\KwOut{$\mathcal{S}$: where $\mathcal{S} = \{C : t \in \mu_M(\sigma_C(R \cup \{t\}))\}$}

\BlankLine

$\mathcal{S} \leftarrow \mathcal{C}^t$;

\ForEach{$t' \in R$}
{
  $\mathcal{R}^{\mathcal{B}^{\mathcal{C}^{t,t'}}} \leftarrow \mathcal{R}^{\mathcal{B}^{\mathcal{C}^{t,t'}}} \cup \{t'\} $;\\
}

\ForEach{$C \in \mathcal{S}$}
{
  \ForEach{$t' \in \mathcal{R}^C$}
  {
    \If{$t' \succ t$}
    {
      $\mathcal{S} \leftarrow \mathcal{S} - \mathcal{C}^{t,t'}$;\\
      \textbf{break} ;
    }
  }
}

$R \leftarrow R \cup \{t\}$;

\Return{$\mathcal{S}$};

\end{algorithm}

==> alg/alg-pullup.tex <==
\begin{algorithm}[t]
\label{alg:pullup}
\caption{Algorithm \algname{pullUp}}
\LinesNumbered
\small

\KwIn{$R(\mathcal{M},\mathcal{D})$: existing tuples; $t$: the new tuple; $U$: set of nodes to pull up;}

\KwOut{$\mathcal{S}$: where $\mathcal{S} = Suprema(\mathcal{C}^{t})$}

\BlankLine

$S \leftarrow \emptyset$;\\
$alreadyVisited \leftarrow false$

\While{$!\ Q.empty()$}
{
	$C \leftarrow Q.dequeue()$;\\
	\If{$C \in U$}
	{
		$alreadyVisited \leftarrow true$;\\
	}		
	$isDominated \leftarrow false$;\\
	\If{$alreadyVisited=false$}
	{
		\ForEach{$t' \in \lambda_M(\sigma_C$ $(R))$}
		{
		    \If{$t \prec t'$}	
		    {
		    	$isDominated \leftarrow true$;\\
		    	\ForEach{$C' \in \mathcal{C}^{t,t'}$}
		    	{
		    			$C'.pruned \leftarrow true$;
		    	}
		    }
		    \ElseIf{$t' \prec t$}
		    {
		    	$\lambda_M(\sigma_C$ $(R)).remove(t')$;\\	
		    	\ForEach{$C' \in \mathcal{CH}^{t'}_C$}
		    	{
		    		\If{$C' \notin \mathcal{C}^{t}$}
		    		{
		    			$\lambda_M(\sigma_{C'}$ $(R)).insert(t')$;
		    		}
		    	}
		    }
		}
	}	
	\If{$(!\ isDominated)\ \&\&\ (!\ C.inserted)$}
	{
		$\lambda_M(\sigma_C$ $(R)).insert(t)$;\\	
		$S \leftarrow S \cup \{C\}$;\\
	}
	\If{$alreadyVisited=false$}
	{
		\ForEach{$C' \in \mathcal{CH}^t_C$}
		{
			\If{$!\ isDominated$}
			{
				$C'.inserted \leftarrow true$;		
			}
			\If{$(!\ Q.contain(C'))\ \&\&\ (! C'.pruned)$}
			{	
				\ForEach{$U' \in U$}
				{
					\If{$C' \in \mathcal{A}_{U'}$}
					{
						$Q.enqueue(C')$;\\
						$break;$\\
					}					
				}					
			}
		}	
	}
}

\Return{$S$};
\end{algorithm}


==> alg/alg-pushdown.tex <==
\begin{algorithm}[t]
\label{alg:pushdown}
\caption{Algorithm \algname{pushDown}}
\LinesNumbered
\small

\KwIn{$R(\mathcal{M},\mathcal{D})$: existing tuples; $t$: the new tuple; $F$: set of nodes to push down;}

\KwOut{$\mathcal{S}$: where $\mathcal{S} = Suprema(\mathcal{C}^{t})$}

\BlankLine

$S \leftarrow \emptyset$;

\ForEach{$N \in \mathcal{CH}_F$}
{
	$\mathcal{Q}.enqueue(N)$;\\
}


\While{$!\ Q.empty()$}
{
$C \leftarrow Q.dequeue()$;\\		
$isDominated \leftarrow false$;\\
\ForEach{$t' \in \lambda_M(\sigma_C$ $(R))$}
{
    \If{$t \prec t'$}	
    {
    	$isDominated \leftarrow true$;\\
    	\ForEach{$C' \in \mathcal{C}^{t,t'}$}
    	{
    			$C'.pruned \leftarrow true$;
    	}
    }
	    \ElseIf{$t' \prec t$}
	    {
	    	$\lambda_M(\sigma_C$ $(R)).remove(t')$;\\	
	    	\ForEach{$C' \in \mathcal{CH}^{t'}_C$}
	    	{
	    		\If{$C' \notin \mathcal{C}^{t}$}
	    		{
	    			$\lambda_M(\sigma_{C'}$ $(R)).insert(t')$;
	    		}
	    	}
	    }
	}
	\If{$(!\ isDominated)\ \&\&\ (!\ C.inserted)$}
	{
		$\lambda_M(\sigma_C$ $(R)).insert(t)$;\\	
		$S \leftarrow S \cup \{C\}$;\\
	}
	\ForEach{$C' \in \mathcal{CH}^t_C$}
	{
		\If{$!\ isDominated$}
		{
			$C'.inserted \leftarrow true$;		
		}
		\If{$(!\ Q.contain(C'))\ \&\&\ (! C'.pruned)$}
		{		
			$Q.enqueue(C')$;
		}
	}
}

\Return{$S$};
\end{algorithm}


==> alg/alg-pushup.tex <==
\begin{algorithm}[t]
\label{algo:pushup}
\caption{pushUp DFS algorithm to discover contextual skylines}
\LinesNumbered

\KwIn{$R$: existing set of tuples; $t$: new tuple; $N$: node to push up; $\mathcal{C}^t$: contextual constraints specific to $t$.}

\KwOut{$\mathcal{S}$: where $\mathcal{S} = \{C : t \in \mu_M(\sigma_C(R \cup \{t\}))\}$}

\BlankLine

$Stack.push(N)$;\\
\While{$Stack.empty()=false$}
{
	$C \leftarrow Stack.pop()$;\\		
	$isDominated \leftarrow false$;\\
	\ForEach{$t' \in \mu_M(\sigma_N$ $(R)$}
	{
	    \If{$t \prec t'$}	
	    {
	    	$isDominated \leftarrow true$;\\
			$break$;
	    }
	    \ElseIf{$t' \prec t$}
	    {
			$\mu_M(\sigma_C$ $(R)).remove(t')$;	
	    }
	}
	\If{$isDominated=false$}
	{
		\If{$C.color=white$}
		{
			$C.color \leftarrow grey$;
			
			\ForEach{$C' \in \mathcal{P}_C[t]$}
			{
				\If{$C'.Color=white$}
				{
					$Stack.push(C')$;
				}
			}
		}
		\ElseIf{$C.Color=grey$}
		{
			$C.Color \leftarrow black$;\\
			$\mu_M(\sigma_C$ $(R)).insert(t)$;\\
			$S \leftarrow S \cup \{C\}$;\\
				
			\ForEach{$C' \in \mathcal{D}_C[t]$}
			{
				$C'.Color \leftarrow blue$;
			}			
		}
	}
}
\Return{$S$};	
\end{algorithm}

==> alg/alg-subspace_sharing.tex <==
\begin{algorithm}[t]
\label{alg:subspace_sharing_distinct_value}
\caption{subspace sharing to minimize computation}
\LinesNumbered

\BlankLine
\tcp{$\psi\ is\ the\ topmost\ node\ of\ skycube$}
$\mathcal{Q}.enqueue(\psi)$;\\
\While{$\mathcal{Q}.empty()=false$}
{
	$M \leftarrow \mathcal{Q}.dequeue()$;\\		
	$Y \leftarrow All\ 0$\\
	\ForEach{$N \in\ Parent(M)$}
	{
		$Y \leftarrow Y \Cap revision(N.X,N.Y)$;
	}	
	$LB_M \leftarrow\ getBoundary(Y)$;
	$LB_M \leftarrow top\_down\_bfs(LB_M,M)$;
	
	\If{$LB_M \neq \phi$}
	{
		\ForEach{$M' \in\ Child(M)$}
		{
			\If{$\mathcal{Q}.contain(M')=false$}
			{
				$\mathcal{Q}.enqueue(M')$;			
			}
		}
	}
}
\end{algorithm}

\begin{algorithm}[t]
\label{alg:intersect}
\caption{$revision(X,Y)$:subspace sharing to minimize computation}
\LinesNumbered

\KwIn{$X,Y$.}

\KwOut{$S \leftarrow X \Cap Y$}

\BlankLine
$Z \leftarrow\ All\ 1$;\\
\For{$i \leftarrow n$}
{
	\If{$X_i=0\ \text{and}\ Y_i=1$}
	{
		$Z' \leftarrow Z$;\\
		$Z'.i \leftarrow 0$;\\
		$S.add(Z')$;
	}
}
\end{algorithm}


==> alg/alg-subspace_sharing_distinct_value.tex <==
\begin{algorithm}[t]
\label{alg:subspace_sharing_distinct_value}
\caption{subspace sharing to minimize computation}
\LinesNumbered

\BlankLine
\tcp{$\psi\ is\ the\ topmost\ node\ of\ skycube$}
$\mathcal{Q}.enqueue(\psi)$;\\
\While{$\mathcal{Q}.empty()=false$}
{
	$M \leftarrow \mathcal{Q}.dequeue()$;\\		
	$LB_M \leftarrow \{\Upsilon\}$;\\
	\ForEach{$N \in\ Parent(M)$}
	{
		$LB_M \leftarrow LB_M \Cap LB_N$;
	}	
	$LB_M \leftarrow top\_down\_bfs(LB_M,M)$;
	
	\If{$LB_M \neq \phi$}
	{
		\ForEach{$M' \in Child(M)$}
		{
			\If{$\mathcal{Q}.contain(M')=false$}
			{
				$\mathcal{Q}.enqueue(M')$;			
			}
		}
	}
}
\end{algorithm}

==> alg/alg-top-down.tex <==
\begin{algorithm}[t]
\label{alg:topdown}
\caption{\algname{TopDown}}
\LinesNumbered
\small

\KwIn{$R(\mathcal{M},\mathcal{D})$: existing tuples; $t$: the new tuple}

\KwOut{$S^t$: the contextual skylines for $t$}

\BlankLine

$S^t \leftarrow \emptyset$;

\ForEach{$M \subseteq \mathcal{M}$}
{
  $S \leftarrow \emptyset$;\\

  \ForEach{$C \in \mathcal{C}^t$}
  {
    $C.\mathit{pruned} \leftarrow \KwSty{false}$;\\
    $C.\mathit{storedInAncestor} \leftarrow \KwSty{false}$;
  }

  $Q.\mathit{enqueue}(\top)$;~\label{line:queueInitTD}\\
  \While{{\bf not} $Q.\mathit{empty}()$}
  {
	$C \leftarrow Q.\mathit{dequeue}()$;\\
	\ForEach{$t' \in \mu_{C,M}$}
	{
	    \If{$t \prec_M t'$}	
	    {
	    	\ForEach{$C' \in \mathcal{C}^{t,t'}$}
	    	{
    			$C'.\mathit{pruned} \leftarrow \KwSty{true}$;
	    	}
	    }
	    \ElseIf{$t' \prec_M t$}
	    {
	    	$\mu_{C,M}.\mathit{remove}(t')$;\\	
	    	\ForEach{$C' \in \mathcal{CH}^{t'}_C-\mathcal{C}^{t}$}
	    	{
		            $\mathit{stored} \leftarrow \KwSty{false}$;\\
	    			\ForEach{$C'' \in \mathcal{A}^{t'}_{C'}-\mathcal{C}^{t}$}
	    			{
	    				\If{$t' \in \mu_{C'',M}$}
	    				{
	    					$\mathit{stored} \leftarrow \KwSty{true}$;\\
	    					\KwSty{break};\\
	    				}
	    			}
	    			\If{{\bf not} $\mathit{stored}$}
	    			{
	    				$\mu_{C',M}.\mathit{insert}(t')$;\\
	    			}	    			
	    	}
	    }
	}
	\If{$(${\bf not} $C.\mathit{pruned})$ {\bf and} $(${\bf not} $C.\mathit{storedInAncestor})$}
	{
		$\mu_{C,M}.\mathit{insert}(t)$;\\	
		$S \leftarrow S \cup \{C\}$;\\
	}
	\ForEach{$C' \in \mathcal{CH}^t_C$}
	{
		\If{{\bf not} $C'.\mathit{pruned}$}
		{
			$C'.\mathit{storedInAncestor} \leftarrow \KwSty{true}$;		
		}
		\If{$(${\bf not} $Q.\mathit{contains}(C'))$}
		{		
			$Q.\mathit{enqueue}(C')$;
		}
	}
  }
  \ForEach{$C \in S$}
  {
    $S^t \leftarrow S^t \cup \{(C,M)\}$;
  }
}
%%%$R \leftarrow R \cup \{t\}$;

\Return{$S^t$};
\end{algorithm}


==> alg/alg-topdown_X_M.tex <==
\begin{algorithm}[t]
\label{algo:Top_down_distinct_value(X, M)}
\caption{$top\_down\_bfs(X,M)$Top-down(X, M) BFS algorithm to discover contextual skylines}
\LinesNumbered

\KwIn{$R$: existing set of tuples; $t$: new tuple; $\mathcal{C}^t$: contextual constraints specific to $t$.}

\KwOut{$\mathcal{S}$: where $\mathcal{S} = Suprema(S')\ and\ \mathcal{S'} = \{C : t \in \mu_M(\sigma_C(R \cup \{t\}))\}$}

\BlankLine

\ForEach{$C_{M'} \in X$}
{
	$\mathcal{Q}.enqueue(C_M)$;
}
\While{$\mathcal{Q}.empty()=false$}
{
	$C \leftarrow \mathcal{Q}.dequeue()$;\\		
	$isDominated \leftarrow false$;\\
	\ForEach{$t' \in \mu_M(\sigma_C$ $(R))$}
	{
	    \If{$t \prec t'$}	
	    {
	    	$isDominated \leftarrow true$;\\
	    	\ForEach{$C' \in \mathcal{D}_C[t]$}
	    	{
	    		\If{$C' \in \mathcal{C}^{t'} $}
	    		{
	    			$C'.pruned \leftarrow true$;
	    		}
	    	}
	    }
	    \ElseIf{$t' \prec t$}
	    {
	    	$\mu_M(\sigma_C$ $(R)).remove(t')$;\\	
	    	\ForEach{$C' \in \mathcal{CH}_C[t']$}
	    	{
	    		\If{$C' \notin \mathcal{C}^{t}$}
	    		{
	    			$\mu_M(\sigma_{C'}$ $(R)).insert(t')$;
	    		}
	    	}
	    }
	}
	\If{$isDominated=false\ \text{and}\ C.inserted=flase$}
	{
		$\mu_M(\sigma_C$ $(R)).insert(t)$;\\	
		$S \leftarrow S \cup \{C\}$;\\		
	}
	\ForEach{$C' \in \mathcal{CH}_C[t]$}
	{
		\If{$isDominated=false$}
		{
			$C'.inserted \leftarrow true$;		
		}
		\If{$\mathcal{Q}.contain(C')=false\ \text{and}\ C'.pruned=false$}
		{		
			$\mathcal{Q}.enqueue(C')$;
		}
	}

}
\Return{$S$};
\end{algorithm}


==> alg/alg-topdown_X_M2.tex <==
\begin{algorithm}[t]
\label{algo:Top_down(X, M)}
\caption{\algname{STopDownNode}}
\LinesNumbered
\small

\KwIn{$R(\mathcal{M},\mathcal{D})$: existing tuples; $t$: the new tuple; $M$: a measure subspace}

\KwOut{$S^t$: the contextual skylines for $t$ in $M$}

\BlankLine

$S^t \leftarrow \emptyset$;

\ForEach{$C \in \mathcal{C}^t$}
{
  $C.pruned \leftarrow false$;\\
  $C.storedInAncestor \leftarrow false$;
}

$Q.enqueue(\top)$;

\While{{\bf not} $Q.empty()$}
{
	$C \leftarrow Q.dequeue()$;	

    %\tcp{\rm deafalt value of $C.marked$ is $false$}
	
	\If{{\bf not} $C.pruned$}
	{
		\ForEach{$t' \in \mu_{C,M}$}
		{
			\If{$t' \prec_M t$}
		    {
		    	$\mu_{C,M}.remove(t')$;
	
	    		\ForEach{$C' \in \mathcal{CH}^{t'}_C-\mathcal{C}^{t}$}
	    		{
	    				$stored \leftarrow false$\\
		    			\ForEach{$C'' \in \mathcal{A}^{t'}_{C'}-\mathcal{C}^{t}$}
		    			{
	    					\If{$t' \in \mu_{C'',M}$}
	    					{
	    						$stored \leftarrow true$;\\
	    						$break$;\\
	    					}
		    			}
		    			\If{\bf{not} $stored$}
	    				{
	    					$\mu_{C',M}.insert(t')$;\\
	    				}	
	    		}
		    }
		}
		\If{{\bf not} $C.storedInAncestor$}
		{
			$\mu_{C,M}.insert(t)$;\\
			$S^t \leftarrow S^t \cup \{(C,M)\}$;	
		}
	}	
	\ForEach{$C' \in \mathcal{CH}^t_C$}
	{
		\If{{\bf not} $C'.pruned$}
		{
			$C'.storedInAncestor \leftarrow true$;		
		}
		\If{$(${\bf not} $Q.contain(C'))$}
		{		
			$Q.enqueue(C')$;
		}
	}
}
\Return{$S^t$};
\end{algorithm}


==> alg/alg-topdown_X_M_distinct_value.tex <==
\begin{algorithm}[t]
\label{algo:Top_down_distinct_value(X, M)}
\caption{$top\_down\_bfs(X,M)$Top-down(X, M) BFS algorithm to discover contextual skylines}
\LinesNumbered

\KwIn{$R$: existing set of tuples; $t$: new tuple; $\mathcal{C}^t$: contextual constraints specific to $t$.}

\KwOut{$\mathcal{S}$: where where $\mathcal{S} = Suprema(S')\ and\ \mathcal{S'} = \{C : t \in \mu_M(\sigma_C(R \cup \{t\}))\}$}

\BlankLine

\ForEach{$C_{M'} \in X$}
{
	$\mathcal{Q}.enqueue(C_M)$;
}
\While{$\mathcal{Q}.empty()=false$}
{
	$C \leftarrow \mathcal{Q}.dequeue()$;\\		
	$isDominated \leftarrow false$;\\
	\ForEach{$t' \in \mu_M(\sigma_C$ $(R))$}
	{
	    \If{$t \prec t'$}	
	    {
	    	$isDominated \leftarrow true$;\\
	    	\ForEach{$C' \in \mathcal{D}_C[t]$}
	    	{
	    		\If{$C' \in \mathcal{C}^{t'} $}
	    		{
	    			$C'.pruned \leftarrow true$;
	    		}
	    	}
	    }
	    \ElseIf{$t' \prec t$}
	    {
	    	$\mu_M(\sigma_C$ $(R)).remove(t')$;\\	
	    	\ForEach{$C' \in \mathcal{CH}_C[t']$}
	    	{
	    		\If{$C' \notin \mathcal{C}^{t}$}
	    		{
	    			$\mu_M(\sigma_{C'}$ $(R)).insert(t')$;\\
   					$S \leftarrow S \cup \{C\}$;\\
	    		}
	    	}
	    }
	}
	\If{$isDominated=false\ \text{and}\ C.inserted=flase$}
	{
		$\mu_M(\sigma_C$ $(R)).insert(t)$;\\	
	}
	\ForEach{$C' \in \mathcal{CH}_C[t]$}
	{
		\If{$isDominated=false$}
		{
			$C'.inserted \leftarrow true$;		
		}
		\If{$\mathcal{Q}.contain(C')=false\ \text{and}\ C'.pruned=false$}
		{		
			$\mathcal{Q}.enqueue(C')$;
		}
	}

}
\Return{$S$};
\end{algorithm}


==> alg/alg-topdown_X_M_version2.tex <==
\begin{algorithm}[t]
\label{algo:Top_down_distinct_value()}
\caption{\algname{STopDownRoot}}
\LinesNumbered
\small

\KwIn{$R(\mathcal{M},\mathcal{D})$: existing tuples; $t$: the new tuple}

\KwOut{$S^t$: the contextual skylines for $t$ in full measure space $\mathcal{M}$}

\BlankLine

$S \leftarrow \emptyset$;

\ForEach{$C \in \mathcal{C}^t$}
{
  $C.pruned \leftarrow false$;\\
  $C.storedInAncestor \leftarrow false$;
}

$Q.enqueue(\top)$;

\While{{\bf not} $Q.empty()$}
{
	$C \leftarrow Q.dequeue()$;\\
	\ForEach{$t' \in \mu(C,\mathcal{M})$}
	{
	    \If{$t \prec_{\mathcal{M}} t'$}	
	    {
	    	\ForEach{$C' \in \mathcal{C}^{t,t'}$}
	    	{
	    		$C'.pruned \leftarrow true$;
	    	}
	    }
	    \ElseIf{$t' \prec_{\mathcal{M}} t$}
	    {
	    	$\mu(C,\mathcal{M}).remove(t')$;\\	
	    	\ForEach{$C' \in \mathcal{CH}^{t'}_C-\mathcal{C}^{t}$}
	    	{
	    			$stored \leftarrow false$;\\
	    			\ForEach{$C'' \in \mathcal{A}^{t'}_{C'}-\mathcal{C}^{t}$}
	    			{
	    				\If{$t' \in \mu(C'',\mathcal{M})$}
	    				{
	    					$stored \leftarrow true$;\\
	    					$break$;\\
	    				}
	    			}
	    			\If{\bf{not} $stored$}
	    			{
	    				$\mu(C',\mathcal{M}).insert(t')$;\\
	    			}	
	    	}
	    }
	    \If{$t' \nprec_{\mathcal{M}} t$}
	    {
	    	\ForEach{$M \subset \mathcal{M}$}
	    	{
	    		\If{$t \prec_{M} t'$}
	    		{
	    			\ForEach{$C' \in \mathcal{C}^{t,t'}$ in subspace $M$}
	    			{
	    				$C'.pruned \leftarrow true$;
	    			}
	    		}
	    	}
	    }
	}
	\If{$(${\bf not} $C.pruned)$ {\bf and} $(${\bf not} $C.storedInAncestor)$}
	{
		$\mu(C,\mathcal{M}).insert(t)$;

        $S \leftarrow S \cup \{C\}$;
	}
	\ForEach{$C' \in \mathcal{CH}^t_C$}
	{
		\If{{\bf not} $C'.pruned$}
		{
			$C'.storedInAncestor \leftarrow true$;		
		}
		\If{$(${\bf not} $Q.contain(C'))$}
		{		
			$Q.enqueue(C')$;
		}
	}
}

$S^t \leftarrow \emptyset$;

\ForEach{$C \in S$}
{
  $S^t \leftarrow S^t \cup \{(C,\mathcal{M})\}$;
}

\Return{$S^t$};
\end{algorithm}


==> alg/alg-topdown_node.tex <==
\begin{algorithm}[t]
\label{algo:Top_down(X, M)}
\caption{\algname{STopDownNode}}
\LinesNumbered
\small

\KwIn{$R(\mathcal{M},\mathcal{D})$: existing tuples; $t$: the new tuple; $M$: a measure subspace}

\KwOut{$S^t$: the contextual skylines for $t$ in $M$}

\BlankLine

$S^t \leftarrow \emptyset$;

\ForEach{$C \in \mathcal{C}^t$}
{
  $C.pruned \leftarrow false$;\\
  $C.storedInAncestor \leftarrow false$;
}

$Q.enqueue(\top)$;

\While{{\bf not} $Q.empty()$}
{
	$C \leftarrow Q.dequeue()$;	

    %\tcp{\rm deafalt value of $C.marked$ is $false$}
	
	\If{{\bf not} $C.pruned$}
	{
		\ForEach{$t' \in \mu_{C,M}$}
		{
			\If{$t' \prec_M t$}
		    {
				\algname{Dominates}$()$;
		    }
		}
		\If{{\bf not} $C.storedInAncestor$}
		{
			$\mu_{C,M}.insert(t)$;\\
			$S^t \leftarrow S^t \cup \{(C,M)\}$;	
		}
	}	
	\algname{EnqueueChindren}$()$;
}
\Return{$S^t$};
\end{algorithm}


==> alg/alg-topdown_root.tex <==
\begin{algorithm}[t]
\label{algo:Top_down_distinct_value()}
\caption{\algname{STopDownRoot}}
\LinesNumbered
\small

\KwIn{$R(\mathcal{M},\mathcal{D})$: existing tuples; $t$: the new tuple}

\KwOut{$S^t$: the contextual skylines for $t$ in full measure space $\mathcal{M}$}

\BlankLine

$S \leftarrow \emptyset$;

\ForEach{$C \in \mathcal{C}^t$}
{
  $C.pruned \leftarrow false$;\\
  $C.storedInAncestor \leftarrow false$;
}

$Q.enqueue(\top)$;

\While{{\bf not} $Q.empty()$}
{
	$C \leftarrow Q.dequeue()$;\\
	\ForEach{$t' \in \mu(C,\mathcal{M})$}
	{
	    \If{$t \prec_{\mathcal{M}} t'$}	
	    {
			\algname{Dominated}$()$;
	    }
	    \ElseIf{$t' \prec_{\mathcal{M}} t$}
	    {
			\algname{Dominates}$()$;
	    }
	    \If{$t' \nprec_{\mathcal{M}} t$}
	    {
	    	\ForEach{$M \subset \mathcal{M}$}
	    	{
	    		\If{$t \prec_{M} t'$}
	    		{
	    			\ForEach{$C' \in \mathcal{C}^{t,t'}$ in subspace $M$}
	    			{
	    				$C'.pruned \leftarrow true$;
	    			}
	    		}
	    	}
	    }
	}
	\If{$(${\bf not} $C.pruned)$ {\bf and} $(${\bf not} $C.storedInAncestor)$}
	{
		$\mu(C,\mathcal{M}).insert(t)$;

        $S \leftarrow S \cup \{C\}$;
	}
	\algname{EnqueueChindren}$()$;
}

$S^t \leftarrow \emptyset$;

\ForEach{$C \in S$}
{
  $S^t \leftarrow S^t \cup \{(C,\mathcal{M})\}$;
}

\Return{$S^t$};
\end{algorithm}


==> naffi-sec-intro.tex <==
It is a basic human instinct that we love to be amazed. And this instinct drives us to scan through the daily newspaper every morning, just to find something new, something interesting. With the advancement of internet, may be the newspaper shifted its place from breakfast table to computer monitor, but our craving for knowing the \textit{``what's new today''} has never diminished rather increased. To satiate this thirst of the reader, journalists and reporters are always busy with finding interesting and significant new facts and presenting as fast as possible. Also the definition of \textit{fastness} has also changed with the flourish of social media and micro blogs. We no longer can patiently wait till next day newspaper comes to know about probable records or significant facts that may happen in tonight's NBA game. To cope with these changes, faster access and advanced operations in data sources are necessary for the journalists. The nascent concept ``Computational Journalism'' focuses on how the power of computation can be leveraged to increase the quality, quantity and effectiveness of journalism.

\begin{comment}
Imagine a world, where you can enjoy a significant fact as it happens in your prefered domain like sports, stock market or even weather before anybody tweets about it. For example, when Michael Jordan just made more than 40 points in three consecutive games or people in Texas feels the highest temperature in its history or IBM becomes one of the companies which is not dominated by any other company in terms of profit margin and dividend yield, you become aware of it. Every event possesses impressiveness, has its own level of significance. All it needs are the proper focus, perspective and appropriate audience for being cherished. Rise of temperature in Texas on a day may not be highest in the history of the world but may be in the history of U.S. or even more specifically in U.S. in 2012. IBM may not be one of the most lucrative stocks in terms of profit margin and dividend yield but may be it is if we also consider net income. So, an event can be significant enough when it is observed from some certain conditions or constraints. It is the art of a journalist to find such conditions and present a fact.\\
\end{comment}

Each and every domain is evolving and being larger; some in higher rate like sports and some in lower rate like government of a country. The problem of discovering and presenting interesting facts from a highly frequently changed domain is tougher and deserves special attention. Here, the response time needs to be faster and more impressive facts or events should get higher priority than less impressive ones. The current world is far from this vision. Currently, investigative journalists use their expertise and knowledge about a domain to find these interesting facts and the conditions where it sounds significant. As there is no systematic approach to discover these facts, journalists and reporters are bound to apply different heuristic and intuition based actions. As a result, the difference between happening of an event and discovering it is quite large. Sometimes there is chance of loosing the freshness and informative quality of the fact. Also, it takes a lot of resources to present interesting and significant facts in reasonable amount of time in absence of a framework. Moreover, chances are there that some significant facts will be missed or some facts will be presented which are not interesting or significant up to par.\reminder{Can we give some evidence that previously some facts were missed and later discovered? Can we also give evidence of some presentation of un-interesting events?}

As we know, there are numerous things which make an event significant. We investigate different properties of significant events. One common property that many significant facts share is they outstand many facts and not get dominated by any fact in their corresponding domain. We can say these are the Skyline of all facts. Specifically, in a dataset containing $m$ numerica attributes, if a tuple is not dominated by any other tuple in all the attributes, we call it a skyline tuple. Fortunately, this concept of Skyline is well studied in database research and there many works to find the skylines of a dataset. In this paper, we work on finding the skyline facts which are significant. The following example will make clearify our goal.

\textbf{\textit{Example:}} In the following table, we have some tuples containing Michael Jordan's performance (points and assists) against Dallas Mavericks and Miami Heats in year 2000 and 2001. If we observe tuple $t_2$, we see that this tuple is the skyline tuple in this small dataset because no other tuple has higher points and assists than this one. So, $t_2$ is obviously a significant fact with respect to this small dataset. Now, consider $t_3$, this is also a significant fact if we consider the records only in year 2000. So, we see that even though $t_3$ does not seem significant with respect to the whole table but it is significant enough when we only consider $year = 2000$. Anoter significance of $t_3$ is, it is also significant when we only consider $opp_{team} = M Heats$ for all years. There is another way to look at the significance of a tuple. A tuple can be significant with respect to some certain measures if not all. For example, $t_5$ is significant if we apply condition $opp_{team} = M Heats$ and consider only $assits$. No other tuple satisfying that condition dominates $t_5$ on $assists$. So, we see that a tuple can be significant in certain conditions and also in certain measures. Suppose a new record $t_n$ is just inserted into the database. To determine whether this fact is significant or not, we need to consider all possible conditions where this tuple may belong and also all possible measure combinations such as <$points$>, <$assists$> and <$points$, $assists$>.

\begin{table}[!ht]
\centering
\caption{Running Example}
\label{tab:running_example}
\begin{tabular}{|l|*{6}{c|}}\hline
id &$player$& $year$ & $team$ & $opp_{team}$ & $points$ & $assists$\\
\hline
\hline
$t_1$ & $M Jordan$ & $2000$ & $C Bulls$ & $D Mavs$ & 10 & 10\\
\hline
$t_2$ & $M Jordan$ & $2001$ & $C Bulls$ & $D Mavs$ & 20 & 14\\
\hline
$t_3$ & $M Jordan$ & $2000$ & $C Bulls$ & $M Heats$ & 15 & 11\\
\hline
$t_4$ & $M Jordan$ & $2001$ & $C Bulls$ & $M Heats$ & 11 & 10\\
\hline
$t_5$ & $M Jordan$ & $2001$ & $C Bulls$ & $M Heats$ & 10 & 12\\
\hline
$t_n$ & $M Jordan$ & $2001$ & $C Bulls$ & $D Mavs$ & 10 & 11\\
\hline
\end{tabular}
\end{table}

In this paper, we investigate the novel problem of automatically finding significant events in a frequently updated domain. Given a database $D$ that is frequently updated with new tuples, whenever a new tuple is inserted into D, we want to identify interesting statements that can be made about the new database state. The challanges and complexities of this problem can be realized if we carefully look at the data and query model. The data model is an append only relational database having many dimensional attributes and many measure attributes. Each dimensional attribute generally have a finite set of values. For example, in the above example, the dimensional attribute team\_name is a set of NBA team names. Another example of dimensional attribute can be season\_year. Here the possible values are calender years like 2010-2011, 2011-2012, etc. The measure attributes generally comprises of numerical values or more specifically ordinal values. The number of plausible significant skyline facts is exponential with respect to number of dimensional and measure attributes. Each unique combination of values from dimensional attributes will create a space for skyline fact. For example, there can be skyline fact for the records having ``Dalls Mavericks'' as team\_name and ``Dirk Nowitzki'' as player name. So it is apparent that there are huge number of combination and thus plausible skyline fact. Moreover, the combination of measure attributes considered makes the problem more challanging. Each combination of measure attributes also provides new skyline.

The query model consists of a new tuple having the same format of the data model. This new tuple, upon insertion, will change the skylines of the combinations which matches with its' dimensinal attribute values. For example, when a new tuple consisting of ``Michael Jordan'' and ``Chicago Bulls'' is inserted into the database, only the dimensinal attribute value combinations having ``Michael Jordan'' or ``Chicago Bulls'' need to be considered for skyline fact discovery. The only exception is the combination which covers all values in all attributes. This is analogous to the concept of empty set being a subset of all possible set. So, the number of combinations to be compared for a single tuple insertion is exponential. Moreover, each dimensinal attribute combination can have exponential number of skyline facts with respect to measure attributes. For a specific dimensional attribute combination, the new tuple  may not be in the skyline considering a subset of the measure attributes but may become significant enough if all the measure attributes are considered. So the search space for significant fact finding is quite formidable.

As mentioned above, in highly frequently updated domains, this skyline change will occur very frequently and significant facts will also occur abundantly. Unless there is a technique to tackle this challange by providing significant facts within reasonable time to the user, the facts will lose their potent.

In our work, we first give a baseline algorithm which is very naive and unreasonably expensive in terms of execution time. This algorithm compares the newly inserted tuple sequentially with all existing tuples and cross out the dimensinal and measure attribute combinations where the new tuple is dominated by the old one. At the end of sequential scan, we only remain with the combinations where the new tuple is in the skyline. We also propose two advanced algorithms based on some prunning properties to solve this problem. In the experiment section, we demonstrate that our advanced algorithm is significantly better than the baseline. We can summarize our contributions in the paper as follows-

\begin{itemize}

\item We formalize the novel problem of significant fact finding. We explain the technical challanges involved and propose solution for them.

\item We develop novel algorithm to approach this problem and compare its performance with baseline.

\item We validate our algorithms over two dataset- NBA boxscore dataset and weather dataset. Our comprehensive experiments show that the algorithms are faster and effective enough to be applied in real life.

\item We propound a threshold based system to identify facts which are more significant and interesting. We also rank the events with respect to their impressiveness.
\end{itemize}

==> sec-alg2.tex <==
\subsection{Frontier Algorithm}\label{sec:alg-frontier}

\begin{definition}[Frontier]
\label{def:frontier}
A lattice of contextual constraints can be divided into two disjoint sets $L1$ and $L2$, where
$L1$ = $\{N|t\notin$ \\ $\mu_{M}(\sigma_N(R))\}$ and $L2$ = $\{N|t\in \mu_{M}(\sigma_N(R))\}$. The set of\\$L2Maxima$ is $L2Maxima$= $\{N|N \subset L2, \nexists N'\in L2\ s.t.\ N' \subset \mathcal{A}_N\}$. The set of $L1Minima$ is $L1Minima$=$\{N|N \subset L1,\nexists N'\in L1\ s.t.\ N \subset \mathcal{A}_{N'}\}$. The set of frontier $L3$ is $L3$ = $L2Maxima \cup \{N|N \subset L2, \exists N'\in L1Mininma\ s. t. (N' \subset \mathcal{A}_N and \nexists N''\in L2Maxima\ s.t.\ \ N' \subset \mathcal{A}_{N''})\}$.\\
\end{definition}

\textit{Example 1: In Figure ~\ref{fig:cuboid}, $L1$ = $\{\perp, a1, c1\}$, $L2$ = $\{b1, a1b1,$ $b1c1, a1c1, a1b1c1\}$. Then corresponding frontier is $L3$=$\{b1,$ $a1c1\}$}.\\

\textit{Example 2: In Figure ~\ref{fig:cuboid}, $L1$ = $\{\perp, a1, c1, a1c1\}$, $L2$ = $\{b1,$ $a1b1, b1c1, a1b1c1\}$. Then corresponding frontier is $L3$=$\{b1,$ $a1c1\}$}.\\

\textit{Example 3: In Figure ~\ref{fig:cuboid}, $L1$ = $\{\perp, a1, b1\}$, $L2$ = $\{c1,a1b1,$ $a1c1,b1c1, a1b1c1\}$. Then corresponding frontier is $L3$=$\{c1, a1b1\}$}.\\

\textit{Example 4: In Figure ~\ref{fig:cuboid}, $L1$ = $\{\perp, a1, b1, a1c1\}$, $L2$ = $\{c1,$ $a1c1,b1c1, a1b1c1\}$. Then corresponding frontier is $L3$=$\{c1, a1b1\}$}.\\

\input{alg/alg-frontier-measure-subspace}
\input{alg/alg-frontier}
\input{alg/alg-pushdown}
\input{alg/alg-pullup}

The basic idea of frontier based algorithm is as follows. Consider new tuple $t$ in measure subspace $M1M2$. Let one of the nodes of its frontier is $D1D2$. Now we need to derive corresponding frontier node for $t$ in $M1M2M3$. If $\exists t' \in D1D2$ such that $t' \succ t$ on $M1M2M3$ (where $t'=t$ on $M1M2$) then there is no such node $X$ in the frontier, such that $X$ is an ancestor of $D1D2$. In this case, the frontier needs to be pushed down. If $\nexists t' \in D1D2$ such that $t' \succ t$ on $M1M2M3$ (where $t'=t$ on $M1M2$) then there is no such node $X$ in the frontier, such that $X$ is an descendant of $D1D2$.$D1D2$ is at least one node of the frontier or a descendant of a frontier node. As for all ancestor $A$ of $D1D2$, $\nexists t'' \in A$ such that $t''\succ t$ or $t''=t$ on $M1M2$ and $t''$ covers $D1D2$. In this case, the frontier is tried to be pulled up. If after pulling up $t$ is dominated by any existing tuple, it needs to be pushed back.\\

Frontier for each measure subspace is computed in Algorithm 9. If the measure subspace representation is power of 2, corresponding frontier is computed by calling Algorithm 5. Otherwise Algorithm 10 is called. The frontier is needed to be reconstructed if it does not cover the parents of $B^{\mathcal{C}^t}$. In Algorithm 10, frontier $F_i$ of a measure subspace $M_i$ is derived based on the frontier $F_{i-1}$ of previous measure subspace $M_{i-1}$. In line 4, all the contextual constraints those belong to $F_{i-1}$ is scanned. In line 6, all the tuples corresponding to those contextual constraints are scanned. In line 16, the contextual constraints where the new tuple $t$ does not got dominated by any other previous tuple is stored in a set $U$. In line 17, Algorithm 12 is called. In line 18, we are calling Algorithm 11.



==> sec-csc.tex <==
\section{CSC}\label{sec:csc}

Xia et al.~\cite{xia2006refreshing} proposed compressed skycube (CSC) to represent the set of measure attributes concisely in a single context. They introduced the concept of minimum subspace. Suppose a tuple $t$ belongs to the skyline of a subspace $U$. If there is no subspace $V$ such that $V \subset U$ where $t$ is in the skyline, then $U$ will be consider as minimum subspace of $t$. Each tuple is stored with respect to its minimum subspaces only. Instead of using all subspaces as cuboid~\cite{PeiYLJELWTYZ06}, CSC only consider a subspace as cuboid if it belongs to minimum  subspaces of any tuple. They have proposed an algorithm to find minimum subspaces. They also proposed another algorithm to answer skyline query (finding skyline tuples for a given subspace $W$). If $X$ is a cuboid in CSC, i.e., $X \subset W$, then the skyline tuples belongs to $X$ are possible candidate for skyline tuples in $U$. After removing the false positives for all such subsets, the exact skyline tuples in $W$ are generated.

Instead of finding answers, our goal is finding queries (finding constraint-measure pairs where a new tuple qualifies as a contextual skyline tuple). In a certain context for finding queries using CSC, we need to find answer for all subspaces. In other word for a new tuple $t$, for each subspace we need to compute whether $t$ belongs to the corresponding skyline. For adapting CSC in our multiple context structure, we need to maintain individual CSC for all possible contexts. We call it Constraint-CSC (\algname{C-CSC}).

In case of \algname{BottomUp} and \algname{TopDown}, storing a tuple and finding corresponding queries are concurrent. On the other hand in \algname{C-CSC}, we need to store a tuple at first and then we can find corresponding queries. While storing, for each tuple $t$ we need to compute minimum subspaces regarding all constraints. Again if a previously stored tuple $t'$ is dominated by $t$, then we need to update the minimum subspaces corresponding to $t'$. In a large dataset where becoming skyline tuple in the subspaces having lower measure attributes is very competitive, finding minimum subspace can be exhaustive. While finding queries, for each constraint we need to check iteratively all the subspaces where $t$ is in the skyline. In a large dataset of many identical valued tuples, a lot of false positives are dealt. There is no sharing along constraints in \algname{C-CSC}. 

==> sec-exp2.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}[b]{.3\textwidth}
   \epsfig{file=images/f8.eps, angle=-90, width=45mm,clip=}
   \caption{Varying $n$, $d$=$7$, $m$=$7$}
\end{subfigure}
\begin{subfigure}[b]{.3\textwidth}
   \epsfig{file=images/f9.eps, angle=-90, width=45mm,clip=}
   \caption{Varying $d$, $n$=$50,000$, $m$=$7$}
\end{subfigure}
\begin{subfigure}[b]{.3\textwidth}
   \epsfig{file=images/f10_.eps, angle=-90, width=45mm,clip=}
   \caption{Varying $m$, $n$=$50,000$, $d$=$7$}
\end{subfigure}
\vspace{-3mm}
\caption{Execution Time of \algname{BaselineSeq}, \algname{BaselineIdx}, \algname{BottomUp} and \algname{TopDown} on the NBA dataset}
\label{fig:BaselineBUTD_}
\end{figure*}

\begin{figure*}[t]
\hspace{-4mm}
\noindent \begin{minipage}{0.75\textwidth}
\centering
\begin{subfigure}[b]{.3\textwidth}
   \epsfig{file=images/f11.eps,angle=-90, width=42mm,clip=}
   \caption{Varying $n$, $d$=$7$, $m$=$7$}
\end{subfigure}
\hspace{1mm}
\begin{subfigure}[b]{.3\textwidth}
   \epsfig{file=images/e5.eps, angle=-90, width=42mm,clip=}
   \caption{Varying $d$, $n$=$50,000$, $m$=$7$}  
\end{subfigure}
\hspace{1mm}
\begin{subfigure}[b]{.3\textwidth}
   \epsfig{file=images/e6.eps, angle=-90, width=42mm,clip=}
   \caption{Varying $m$, $n$=$50,000$, $d$=$7$}   
\end{subfigure}
\hspace{1mm}
\caption{Execution Time of \algname{BottomUp}, \algname{TopDown}, \algname{SBottomUp} and \algname{STopDown} on the NBA dataset}
\end{minipage}
\noindent \begin{minipage}{0.27\textwidth}
\centering
\epsfig{file=images/f14.eps, angle=-90, width=42mm,clip=}\vspace{-2mm}
\caption{Execution Time of \algname{BottomUp}, \algname{TopDown}, \algname{SBottomUp} and \algname{STopDown} on the Weather Dataset, Varying $n$, $d$=$7$, $m$=$7$}
\end{minipage}
\vspace{-3mm}
\end{figure*}

\begin{figure}[t]
\begin{subfigure}[b]{.5\linewidth}
   \epsfig{file=images/f15.eps, angle=-90, width=40mm,clip=}
   \caption{Size of Consumed Memory}
\end{subfigure}
\begin{subfigure}[b]{.5\linewidth}
   \epsfig{file=images/f16.eps, angle=-90, width=40mm,clip=}
   \caption{Number of Skyline Tuples Stored}
\end{subfigure}
   \vspace{-3mm}
\caption{Memory Consumption by \algname{BottomUp}, \algname{TopDown}, \algname{SBottomUp} and \algname{STopDown} on the NBA Dataset, Varying $n$, $d$=$7$, $m$=$7$}
\end{figure}

\begin{figure}[t]
\begin{subfigure}[b]{.5\linewidth}
   \epsfig{file=images/c_id.eps, angle=-90, width=40mm,clip=}
   \caption{Number of Comparisons}
   \label{fig:c_id}
\end{subfigure}
\begin{subfigure}[b]{.5\linewidth}
   \epsfig{file=images/t_id.eps, angle=-90, width=40mm,clip=}
   \caption{Number of Traversed Constraints}
   \label{fig:t_id}
\end{subfigure}
   \vspace{-3mm}
\caption{Work Done by \algname{BottomUp}, \algname{TopDown}, \algname{SBottomUp} and \algname{STopDown} on the NBA Dataset, Varying $n$, $d$=$7$, $m$=$7$}
\label{fig:work_}
\end{figure}

\begin{figure*}[t]
\hspace{-4mm}
\noindent \begin{minipage}{0.75\textwidth}
\centering
\begin{subfigure}[b]{.3\textwidth}
   \epsfig{file=images/f17.eps, angle=-90, width=42mm,clip=}
   \caption{Varying $n$, $d$=$7$, $m$=$7$}
\end{subfigure}
\hspace{1mm}
\begin{subfigure}[b]{.3\textwidth}
   \epsfig{file=images/time_d_f2.eps, angle=-90, width=42mm,clip=}
   \caption{Varying $d$, $n$=$100$, $m$=$7$}
\end{subfigure}
\hspace{1mm}
\begin{subfigure}[b]{.3\textwidth}
   \epsfig{file=images/time_m_f3.eps, angle=-90, width=42mm,clip=}
   \caption{Varying $m$, $n$=$100$, $d$=$7$}
  \end{subfigure}
\caption{Execution Time of \algname{FSBottomUp} and \algname{FSTopDown} on the NBA Dataset}
\end{minipage}
\noindent \begin{minipage}{0.27\textwidth}
\centering
\epsfig{file=images/time_id_f4.eps, angle=-90, width=42mm,clip=}\vspace{-2mm}
\caption{Execution Time of \algname{FSBottomUp} and \algname{FSTopDown} on the Weather Dataset, Varying $n$, $d$=$7$, $m$=$7$}
\end{minipage}
\vspace{-3mm}
\end{figure*}
%Figure~\ref{fig:time_id_b} compares the execution times (in logarithmic scale) of \algname{BaselineSeq}, \algname{BaselineIdx}, \algname{BottomUp} and \algname{TopDown} on the NBA dataset. Figure~\ref{fig:time_id_5_7} and Figure~\ref{fig:time_id_5_7_weather} compare the execution times of \algname{BottomUp}, \algname{TopDown}, \algname{SBottomUp} and \algname{STopDown} on the NBA dataset and Weather dataset, respectively. For these three figures, $d$=$7$ and $m$=$7$. We observed that though the performance of \algname{STopDown} over \algname{TopDown} is substantially better, \algname{SBottomUp} is not that better in comparison with \algname{BottomUp}. Here is an explanation of the reason. Suppose a new tuple $t$ compared with $t$ in $\mu_{C,\mathcal{M}}$ and according to subspace sharing in \algname{SBottomUp} we get that $t$ will not be in the skyline of $\mu_{C',M}$, $C' \in C \cup \mathcal{A}^t_C$. On the other hand, in \algname{BottomUp} we need to compare $t$ with the content of $\mu_{C,M}$ to prune $\mu_{C',M}$, $C' \in C \cup \mathcal{A}^t_C$. We can see that using \algname{SBottomUp} comparison regarding only one constraint is skipped. As \algname{TopDown} needs to go through every constraint, in \algname{STopDown} discarding $\mathcal{C}^{t,t'}$ saves a lot.

%Figure~\ref{fig:c_id} compare the number of comparisons in \algname{BottomUp}, \algname{TopDown}, \algname{SBottomUp} and \algname{STopDown} on the NBA dataset. Figure~\ref{fig:t_id} compare the number of traversed constraints in \algname{BottomUp}, \algname{TopDown}, \algname{SBottomUp} and \algname{STopDown} on the NBA dataset. For both figures, $d$=$7$ and $m$=$7$.

